Cylindrical Battery Fault Detection under Extreme Fast Charging: A Physics-based Learning Approach

High power operation in extreme fast charging significantly increases the risk of internal faults in Electric Vehicle batteries which can lead to accelerated battery failure. Early detection of these faults is crucial for battery safety and widespread deployment of fast charging. In this setting, we propose a real-time {detection} framework for battery voltage and thermal faults. A major challenge in battery fault detection arises from the effect of uncertainties originating from sensor inaccuracies, nominal aging, or unmodelled dynamics. Inspired by physics-based learning, we explore a detection paradigm that combines physics-based models, model-based detection observers, and data-driven learning techniques to address this challenge. Specifically, we construct the {detection} observers based on an experimentally identified electrochemical-thermal model, and subsequently design the observer tuning parameters following Lyapunov's stability theory. Furthermore, we utilize Gaussian Process Regression technique to learn the model and measurement uncertainties which in turn aid the {detection} observers in distinguishing faults and uncertainties. Such uncertainty learning essentially helps suppressing their effects, potentially enabling early detection of faults. We perform simulation and experimental case studies on the proposed fault {detection} scheme verifying the potential of physics-based learning in early detection of battery faults.

==> Bibliography/Bibfilev2.tex <==
@article{wandt2018quantitative,
  title={Quantitative and time-resolved detection of lithium plating on graphite anodes in lithium ion batteries},
  author={Wandt, Johannes and Jakes, Peter and Granwehr, Josef and Eichel, R{\"u}diger-A and Gasteiger, Hubert A},
  journal={Materials Today},
  volume={21},
  number={3},
  pages={231--240},
  year={2018},
  publisher={Elsevier}
}

@article{lee2021convolutional,
  title={Convolutional Neural Network-Based False Battery Data Detection and Classification for Battery Energy Storage Systems},
  author={Lee, Hyunjun and Kim, Kyungtak and Park, Joung-Hu and Bere, Gomanth and Ochoa, Justin Joshua and Kim, Taesic},
  journal={IEEE Transactions on Energy Conversion},
  year={2021},
  publisher={IEEE}
}

@article{schmid2020data,
  title={{Data-Driven Fault Diagnosis in Battery Systems through Cross-Cell Monitoring}},
  author={Schmid, Michael and Kneidinger, Hans-Georg and Endisch, Christian},
  journal={IEEE Sensors Journal},
  year={2020},
  publisher={IEEE}
}

@article{shang2020multi,
  title={{A multi-fault diagnosis method based on modified Sample Entropy for lithium-ion battery strings}},
  author={Shang, Yunlong and Lu, Gaopeng and Kang, Yongzhe and Zhou, Zhongkai and Duan, Bin and Zhang, Chenghui},
  journal={Journal of Power Sources},
  volume={446},
  pages={227275},
  year={2020},
  publisher={Elsevier}
}

@article{xiong2020research,
  title={{Research progress, challenges and prospects of fault diagnosis on battery system of electric vehicles}},
  author={Xiong, Rui and Sun, Wanzhou and Yu, Quanqing and Sun, Fengchun},
  journal={Applied Energy},
  volume={279},
  pages={115855},
  year={2020},
  publisher={Elsevier}
}

@article{yao2020novel,
  title={{A novel intelligent method for fault diagnosis of electric vehicle battery system based on wavelet neural network}},
  author={Yao, Lei and Xiao, Yanqiu and Gong, Xiaoyun and Hou, Junjian and Chen, Xiangtian},
  journal={Journal of Power Sources},
  volume={453},
  pages={227870},
  year={2020},
  publisher={Elsevier}
}

@article{li2020battery,
  title={{Battery Fault Diagnosis for Electric Vehicles Based on Voltage Abnormality by Combining the Long Short-Term Memory Neural Network and the Equivalent Circuit Model}},
  author={Li, Da and Zhang, Zhaosheng and Liu, Peng and Wang, Zhenpo and Zhang, Lei},
  journal={IEEE Transactions on Power Electronics},
  volume={36},
  number={2},
  pages={1303--1315},
  year={2020},
  publisher={IEEE}
}

@article{hu2020advanced,
  title={{Advanced Fault Diagnosis for Lithium-Ion Battery Systems: A Review of Fault Mechanisms, Fault Features, and Diagnosis Procedures}},
  author={Hu, Xiaosong and Zhang, Kai and Liu, Kailong and Lin, Xianke and Dey, Satadru and Onori, Simona},
  journal={IEEE Industrial Electronics Magazine},
  volume={14},
  number={3},
  pages={65--91},
  year={2020},
  publisher={IEEE}
}

@article{finegan2020application,
  title={ {The Application of Data-Driven Methods and Physics-Based Learning for Improving Battery Safety}},
  author={Finegan, Donal P and Zhu, Juner and Feng, Xuning and Keyser, Matt and Ulmefors, Marcus and Li, Wei and Bazant, Martin Z and Cooper, Samuel J},
  journal={Joule},
  year={2020},
  publisher={Elsevier}
}

@article{zhang2002robust,
  title={ {A robust detection and isolation scheme for abrupt and incipient faults in nonlinear systems}},
  author={Zhang, Xiaodong and Polycarpou, Marios M and Parisini, Thomas},
  journal={IEEE transactions on automatic control},
  volume={47},
  number={4},
  pages={576--593},
  year={2002},
  publisher={IEEE}
}

@article{zhong2003lmi,
  title={ {An LMI approach to design robust fault detection filter for uncertain LTI systems}},
  author={Zhong, Maiying and Ding, Steven X and Lam, James and Wang, Haibo},
  journal={Automatica},
  volume={39},
  number={3},
  pages={543--550},
  year={2003},
  publisher={Elsevier}
}

@article{tomaszewska2019lithium,
  title={ {Lithium-ion battery fast charging: a review}},
  author={Tomaszewska, Anna and Chu, Zhengyu and Feng, Xuning and O'Kane, Simon and Liu, Xinhua and Chen, Jingyi and Ji, Chenzhen and Endler, Elizabeth and Li, Ruihe and Liu, Lishuo and others},
  journal={ETransportation},
  volume={1},
  pages={100011},
  year={2019},
  publisher={Elsevier}
}

@article{ahmed2017enabling,
  title={ {Enabling fast charging--A battery technology gap assessment}},
  author={Ahmed, Shabbir and Bloom, Ira and Jansen, Andrew N and Tanim, Tanvir and Dufek, Eric J and Pesaran, Ahmad and Burnham, Andrew and Carlson, Richard B and Dias, Fernando and Hardy, Keith and others},
  journal={Journal of Power Sources},
  volume={367},
  pages={250--262},
  year={2017},
  publisher={Elsevier}
}

@article{guo2011thermal,
  title={Thermal model for lithium ion battery pack with mixed parallel and series configuration},
  author={Guo, Meng and White, Ralph E},
  journal={Journal of the Electrochemical Society},
  volume={158},
  number={10},
  pages={A1166},
  year={2011},
  publisher={IOP Publishing}
}

@inproceedings{rasmussen2003gaussian,
  title={Gaussian processes in machine learning},
  author={Rasmussen, Carl Edward},
  booktitle={Summer School on Machine Learning},
  pages={63--71},
  year={2003},
  organization={Springer}
}

@article{recht2019tour,
  title={A tour of reinforcement learning: The view from continuous control},
  author={Recht, Benjamin},
  journal={Annual Review of Control, Robotics, and Autonomous Systems},
  volume={2},
  pages={253--279},
  year={2019},
  publisher={Annual Reviews}
}

@inproceedings{berkenkamp2015safe,
  title={Safe and robust learning control with Gaussian processes},
  author={Berkenkamp, Felix and Schoellig, Angela P},
  booktitle={2015 European Control Conference (ECC)},
  pages={2496--2501},
  year={2015},
  organization={IEEE}
}

@article{zhang2018long,
  title={Long short-term memory recurrent neural network for remaining useful life prediction of lithium-ion batteries},
  author={Zhang, Yongzhi and Xiong, Rui and He, Hongwen and Pecht, Michael G},
  journal={IEEE Transactions on Vehicular Technology},
  volume={67},
  number={7},
  pages={5695--5705},
  year={2018},
  publisher={IEEE}
}

@article{nuhic2013health,
  title={Health diagnosis and remaining useful life prognostics of lithium-ion batteries using data-driven methods},
  author={Nuhic, Adnan and Terzimehic, Tarik and Soczka-Guth, Thomas and Buchholz, Michael and Dietmayer, Klaus},
  journal={Journal of power sources},
  volume={239},
  pages={680--688},
  year={2013},
  publisher={Elsevier}
}

@article{zhao2017fault,
  title={Fault and defect diagnosis of battery for electric vehicles based on big data analysis methods},
  author={Zhao, Yang and Liu, Peng and Wang, Zhenpo and Zhang, Lei and Hong, Jichao},
  journal={Applied Energy},
  volume={207},
  pages={354--362},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{dey2015diagnostic,
  title={A diagnostic scheme for detection, isolation and estimation of electrochemical faults in lithium-ion cells},
  author={Dey, Satadru and Ayalew, Beshah},
  booktitle={ASME 2015 Dynamic Systems and Control Conference},
  year={2015},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@article{dey2017model,
  title={Model-based battery thermal fault diagnostics: Algorithms, analysis, and experiments},
  author={Dey, Satadru and Perez, Hector E and Moura, Scott J},
  journal={IEEE Transactions on Control Systems Technology},
  volume={27},
  number={2},
  pages={576--587},
  year={2017},
  publisher={IEEE}
}

@article{ALHALLAJ19991,
title = "Thermal modeling and design considerations of lithium-ion batteries",
journal = "Journal of Power Sources",
volume = "83",
number = "1",
pages = "1 - 8",
year = "1999",
author = "S. Al Hallaj and H. Maleki and J.S. Hong and J.R. Selman",
}

@ARTICLE{7004795,
author={S. {Dey} and B. {Ayalew} and P. {Pisu}},
journal={IEEE Transactions on Control Systems Technology},
title={Nonlinear Robust Observers for State-of-Charge Estimation of Lithium-Ion Cells Based on a Reduced Electrochemical Model},
year={2015},
volume={23},
number={5},
pages={1935-1942},}


@article{santhanagopalan2006online,
  title={Online estimation of the state of charge of a lithium ion cell},
  author={Santhanagopalan, Shriram and White, Ralph E},
  journal={Journal of power sources},
  volume={161},
  number={2},
  pages={1346--1355},
  year={2006},
  publisher={Elsevier}
}

@article{sidhu2014adaptive,
  title={Adaptive nonlinear model-based fault diagnosis of Li-ion batteries},
  author={Sidhu, Amardeep and Izadian, Afshin and Anwar, Sohel},
  journal={IEEE Transactions on Industrial Electronics},
  volume={62},
  number={2},
  pages={1002--1011},
  year={2014},
  publisher={IEEE}
}

@inproceedings{marcicki2010nonlinear,
  title={Nonlinear fault detection and isolation for a lithium-ion battery management system},
  author={Marcicki, Jim and Onori, Simona and Rizzoni, Giorgio},
  booktitle={ASME 2010 Dynamic Systems and Control Conference},
  pages={607--614},
  year={2010},
  organization={American Society of Mechanical Engineers Digital Collection}
}


@article{bandhauer2011critical,
  title={A critical review of thermal issues in lithium-ion batteries},
  author={Bandhauer, Todd M and Garimella, Srinivas and Fuller, Thomas F},
  journal={Journal of the Electrochemical Society},
  volume={158},
  number={3},
  pages={R1--R25},
  year={2011},
  publisher={The Electrochemical Society}
}

@article{doughty2012general,
  title={A general discussion of Li ion battery safety},
  author={Doughty, Daniel H and Roth, E Peter},
  journal={The Electrochemical Society Interface},
  volume={21},
  number={2},
  pages={37--44},
  year={2012},
  publisher={The Electrochemical Society}
}

@article{liu2016understanding,
  title={Understanding undesirable anode lithium plating issues in lithium-ion batteries},
  author={Liu, Qianqian and Du, Chunyu and Shen, Bin and Zuo, Pengjian and Cheng, Xinqun and Ma, Yulin and Yin, Geping and Gao, Yunzhi},
  journal={RSC Advances},
  volume={6},
  number={91},
  pages={88683--88700},
  year={2016},
  publisher={Royal Society of Chemistry}
}

@article{bugga2010lithium,
  title={Lithium plating behavior in lithium-ion cells},
  author={Bugga, Ratnakumar V and Smart, Marshall C},
  journal={ECS Transactions},
  volume={25},
  number={36},
  pages={241--252},
  year={2010},
  publisher={The Electrochemical Society}
}

@article{yao2015fault,
  title={Fault detection of the connection of lithium-ion power batteries based on entropy for electric vehicles},
  author={Yao, Lei and Wang, Zhenpo and Ma, Jun},
  journal={Journal of Power Sources},
  volume={293},
  pages={548--561},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{saha2008uncertainty,
  title={Uncertainty management for diagnostics and prognostics of batteries using Bayesian techniques},
  author={Saha, Bhaskar and Goebel, Kai},
  booktitle={2008 IEEE Aerospace Conference},
  pages={1--8},
  year={2008},
  organization={IEEE}
}

@article{xiong2019online,
  title={Online Fault Diagnosis of External Short Circuit for Lithium-ion Battery Pack},
  author={Xiong, Rui and Yang, Ruixin and Chen, Zeyu and Shen, Weixiang and Sun, Fengchun},
  journal={IEEE Transactions on Industrial Electronics},
  year={2019},
  publisher={IEEE}
}

@article{wei2019lyapunov,
  title={Lyapunov-based thermal fault diagnosis of cylindrical lithium-ion batteries},
  author={Wei, Jingwen and Dong, Guangzhong and Chen, Zonghai},
  journal={IEEE Transactions on Industrial Electronics},
  year={2019},
  publisher={IEEE}
}

@inproceedings{liu2014fault,
  title={Fault detection and isolation for lithium-ion battery system using structural analysis and sequential residual generation},
  author={Liu, Zhentong and Ahmed, Qadeer and Rizzoni, Giorgio and He, Hongwen},
  booktitle={ASME 2014 dynamic systems and control conference},
  year={2014},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@article{di2010lithium,
  title={Lithium-ion battery state of charge and critical surface charge estimation using an electrochemical model-based extended Kalman filter},
  author={Di Domenico, Domenico and Stefanopoulou, Anna and Fiengo, Giovanni},
  journal={Journal of dynamic systems, measurement, and control},
  volume={132},
  number={6},
  pages={061302},
  year={2010},
  publisher={American Society of Mechanical Engineers}
}

@article{birkl2017degradation,
  title={Degradation diagnostics for lithium ion cells},
  author={Birkl, Christoph R and Roberts, Matthew R and McTurk, Euan and Bruce, Peter G and Howey, David A},
  journal={Journal of Power Sources},
  volume={341},
  pages={373--386},
  year={2017},
  publisher={Elsevier}
}

@article{dubarry2012synthesize,
  title={Synthesize battery degradation modes via a diagnostic and prognostic model},
  author={Dubarry, Matthieu and Truchot, Cyril and Liaw, Bor Yann},
  journal={Journal of power sources},
  volume={219},
  pages={204--216},
  year={2012},
  publisher={Elsevier}
}

@article{moura2014adaptive,
  title={Adaptive partial differential equation observer for battery state-of-charge/state-of-health estimation via an electrochemical model},
  author={Moura, Scott J and Chaturvedi, Nalin A and Krsti{\'c}, Miroslav},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={136},
  number={1},
  pages={011015},
  year={2014},
  publisher={American Society of Mechanical Engineers}
}

@article{dey2015nonlinear,
  title={Nonlinear robust observers for state-of-charge estimation of lithium-ion cells based on a reduced electrochemical model},
  author={Dey, Satadru and Ayalew, Beshah and Pisu, Pierluigi},
  journal={IEEE Transactions on Control Systems Technology},
  volume={23},
  number={5},
  pages={1935--1942},
  year={2015},
  publisher={IEEE}
}

@inproceedings{ebbesen2012generic,
  title={A generic particle swarm optimization Matlab function},
  author={Ebbesen, Soren and Kiwitz, Pascal and Guzzella, Lino},
  booktitle={American Control Conference (ACC), 2012},
  pages={1519--1524},
  year={2012},
  organization={IEEE}
}

@article{cho1997systematic,
  title={A systematic approach to adaptive observer synthesis for nonlinear systems},
  author={Cho, Young Man and Rajamani, Rajesh},
  journal={IEEE transactions on Automatic Control},
  volume={42},
  number={4},
  pages={534--537},
  year={1997},
  publisher={IEEE}
}

@article{khalil2002nonlinear,
  title={Nonlinear systems, 3rd},
  author={Khalil, Hassan K},
  journal={New Jewsey, Prentice Hall},
  volume={9},
  number={4.2},
  year={2002}
}

@article{broussely2005main,
  title={Main aging mechanisms in Li ion batteries},
  author={Broussely, Michel and Biensan, Ph and Bonhomme, F and Blanchard, Ph and Herreyre, S and Nechev, K and Staniewicz, RJ},
  journal={Journal of power sources},
  volume={146},
  number={1-2},
  pages={90--96},
  year={2005},
  publisher={Elsevier}
}

@article{bartlett2016electrochemical,
  title={Electrochemical model-based state of charge and capacity estimation for a composite electrode lithium-ion battery},
  author={Bartlett, Alexander and Marcicki, James and Onori, Simona and Rizzoni, Giorgio and Yang, Xiao Guang and Miller, Ted},
  journal={IEEE Transactions on Control Systems Technology},
  volume={24},
  number={2},
  pages={384--399},
  year={2016},
  publisher={IEEE}
}

@article{dey2017real,
  title={Real-Time Estimation of Lithium-Ion Concentration in Both Electrodes of a Lithium-Ion Battery Cell Utilizing Electrochemical--Thermal Coupling},
  author={Dey, Satadru and Ayalew, Beshah},
  journal={Journal of Dynamic Systems, Measurement, and Control},
  volume={139},
  number={3},
  pages={031007},
  year={2017},
  publisher={American Society of Mechanical Engineers}
}

@article{allam2018interconnected,
  title={An Interconnected Observer for Concurrent Estimation of Bulk and Surface Concentration in Cathode and Anode of a Lithium-ion Battery},
  author={Allam, Anirudh and Onori, Simona},
  journal={IEEE Transactions on Industrial Electronics},
  year={2018},
  publisher={IEEE}
}

@article{moura2017battery,
  title={Battery state estimation for a single particle model with electrolyte dynamics},
  author={Moura, Scott J and Argomedo, Federico Bribiesca and Klein, Reinhardt and Mirtabatabaei, Anahita and Krstic, Miroslav},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={2},
  pages={453--468},
  year={2017},
  publisher={IEEE}
}

@article{plett2004extended,
  title={Extended Kalman filtering for battery management systems of LiPB-based HEV battery packs: Part 3. State and parameter estimation},
  author={Plett, Gregory L},
  journal={Journal of Power sources},
  volume={134},
  number={2},
  pages={277--292},
  year={2004},
  publisher={Elsevier}
}

@article{kim2010technique,
  title={A technique for estimating the state of health of lithium batteries through a dual-sliding-mode observer},
  author={Kim, IL-Song},
  journal={IEEE Transactions on Power Electronics},
  volume={25},
  number={4},
  pages={1013--1022},
  year={2010},
  publisher={IEEE}
}

@article{smith2010model,
  title={Model-based electrochemical estimation and constraint management for pulse operation of lithium ion batteries},
  author={Smith, Kandler A and Rahn, Christopher D and Wang, Chao-Yang},
  journal={IEEE Transactions on Control Systems Technology},
  volume={18},
  number={3},
  pages={654--663},
  year={2010},
  publisher={IEEE}
}

@article{charkhgard2010state,
  title={State-of-charge estimation for lithium-ion batteries using neural networks and EKF},
  author={Charkhgard, Mohammad and Farrokhi, Mohammad},
  journal={IEEE transactions on industrial electronics},
  volume={57},
  number={12},
  pages={4178--4187},
  year={2010},
  publisher={IEEE}
}

@article{chaoui2015lyapunov,
  title={Lyapunov-based adaptive state of charge and state of health estimation for lithium-ion batteries},
  author={Chaoui, Hicham and Golbon, Navid and Hmouz, Imad and Souissi, Ridha and Tahar, Sofi{\`e}ne},
  journal={IEEE Transactions on Industrial Electronics},
  volume={62},
  number={3},
  pages={1610--1618},
  year={2015},
  publisher={IEEE}
}

@article{rahimi2014online,
  title={Online adaptive parameter identification and state-of-charge coestimation for lithium-polymer battery cells},
  author={Rahimi-Eichi, Habiballah and Baronti, Federico and Chow, Mo-Yuen},
  journal={IEEE Transactions on Industrial Electronics},
  volume={61},
  number={4},
  pages={2053--2061},
  year={2014},
  publisher={IEEE}
}

@article{santhanagopalan2006online,
  title={Online estimation of the state of charge of a lithium ion cell},
  author={Santhanagopalan, Shriram and White, Ralph E},
  journal={Journal of power sources},
  volume={161},
  number={2},
  pages={1346--1355},
  year={2006},
  publisher={Elsevier}
}

@article{lotfi2017reduced,
  title={Reduced-order electrochemical model-based soc observer with output model uncertainty estimation},
  author={Lotfi, Nima and Landers, Robert G and Li, Jie and Park, Jonghyun},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={4},
  pages={1217--1230},
  year={2017},
  publisher={IEEE}
}

@article{wang2015adaptive,
  title={Adaptive estimation of the state of charge for lithium-ion batteries: Nonlinear geometric observer approach},
  author={Wang, Yebin and Fang, Huazhen and Sahinoglu, Zafer and Wada, Toshihiro and Hara, Satoshi},
  journal={IEEE Transactions on Control Systems Technology},
  volume={23},
  number={3},
  pages={948--962},
  year={2015},
  publisher={IEEE}
}

@article{tanim2015state,
  title={State of charge estimation of a lithium ion cell based on a temperature dependent and electrolyte enhanced single particle model},
  author={Tanim, Tanvir R and Rahn, Christopher D and Wang, Chao-Yang},
  journal={Energy},
  volume={80},
  pages={731--739},
  year={2015},
  publisher={Elsevier}
}

@article{gholizadeh2014estimation,
  title={Estimation of state of charge, unknown nonlinearities, and state of health of a lithium-ion battery based on a comprehensive unobservable model},
  author={Gholizadeh, Mehdi and Salmasi, Farzad R},
  journal={IEEE Transactions on Industrial Electronics},
  volume={61},
  number={3},
  pages={1335--1344},
  year={2014},
  publisher={IEEE}
}

@article{saha2009prognostics,
  title={Prognostics methods for battery health monitoring using a Bayesian framework},
  author={Saha, Bhaskar and Goebel, Kai and Poll, Scott and Christophersen, Jon},
  journal={IEEE Transactions on instrumentation and measurement},
  volume={58},
  number={2},
  pages={291--296},
  year={2009},
  publisher={IEEE}
}

@book{smyshlyaev2010adaptive,
  title={Adaptive control of parabolic PDEs},
  author={Smyshlyaev, Andrey and Krstic, Miroslav},
  year={2010},
  publisher={Princeton University Press}
}














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



@Manual{website2017,
title = {Pump up the Charge with Extreme Fast Charging},
author = {Chehab, Nay},    
note = {Available at {https://energy.gov/eere/articles/pump-charge-extreme-fast-charging}}
}
@book{andrea2010battery,
  title={Battery management systems for large lithium-ion battery packs},
  author={Andrea, Davide},
  year={2010},
  publisher={Artech house}
}
@article{zhang2006effect,
  title={The effect of the charging protocol on the cycle life of a Li-ion battery},
  author={Zhang, Sheng Shui},
  journal={Journal of power sources},
  volume={161},
  number={2},
  pages={1385--1391},
  year={2006},
  publisher={Elsevier}
}
@article{liu2011search,
  title={Search for an optimal five-step charging pattern for Li-ion batteries using consecutive orthogonal arrays},
  author={Liu, Yi-Hwa and Hsieh, Ching-Hsing and Luo, Yi-Feng},
  journal={IEEE Transactions on Energy Conversion},
  volume={26},
  number={2},
  pages={654--661},
  year={2011},
  publisher={IEEE}
}
@article{abdel2017influence,
  title={Influence analysis of static and dynamic fast-charging current profiles on ageing performance of commercial lithium-ion batteries},
  author={Abdel-Monem, Mohamed and Trad, Khiem and Omar, Noshin and Hegazy, Omar and Van den Bossche, Peter and Van Mierlo, Joeri},
  journal={Energy},
  volume={120},
  pages={179--191},
  year={2017},
  publisher={Elsevier}
}
@article{ullah1996fast,
  title={Fast intelligent battery charging: neural-fuzzy approach},
  author={Ullah, Zafar and Burford, Brian and Dillip, S},
  journal={IEEE Aerospace and Electronic Systems Magazine},
  volume={11},
  number={6},
  pages={26--34},
  year={1996},
  publisher={IEEE}
}

@article{surmann1996genetic,
  title={Genetic optimization of a fuzzy system for charging batteries},
  author={Surmann, Hartmut},
  journal={IEEE Transactions on Industrial Electronics},
  volume={43},
  number={5},
  pages={541--548},
  year={1996},
  publisher={IEEE}
}
@article{liu2005search,
  title={Search for an optimal rapid charging pattern for lithium-ion batteries using ant colony system algorithm},
  author={Liu, Yi-Hwa and Teng, Jen-Hao and Lin, Yu-Chung},
  journal={IEEE Transactions on Industrial Electronics},
  volume={52},
  number={5},
  pages={1328--1336},
  year={2005},
  publisher={IEEE}
}
@book{lewis2012optimal,
  title={Optimal control},
  author={Lewis, Frank L and Vrabie, Draguna and Syrmos, Vassilis L},
  year={2012},
  publisher={John Wiley \& Sons}
}
@article{chen2008design,
  title={A design of a grey-predicted Li-ion battery charge system},
  author={Chen, Liang-Rui and Hsu, Roy Chaoming and Liu, Chuan-Sheng},
  journal={IEEE Transactions on Industrial Electronics},
  volume={55},
  number={10},
  pages={3692--3701},
  year={2008},
  publisher={IEEE}
}
@inproceedings{parvini2015maximizing,
  title={Maximizing charging efficiency of lithium-ion and lead-acid batteries using optimal control theory},
  author={Parvini, Yasha and Vahidi, Ardalan},
  booktitle={American Control Conference (ACC), 2015},
  pages={317--322},
  year={2015},
  organization={IEEE}
}
@article{abdollahi2016optimal,
  title={Optimal battery charging, Part I: Minimizing time-to-charge, energy loss, and temperature rise for OCV-resistance battery model},
  author={Abdollahi, A and Han, X and Avvari, GV and Raghunathan, N and Balasingam, B and Pattipati, KR and Bar-Shalom, Y},
  journal={Journal of Power Sources},
  volume={303},
  pages={388--398},
  year={2016},
  publisher={Elsevier}
}
@article{chu2017non,
  title={Non-destructive fast charging algorithm of lithium-ion batteries based on the control-oriented electrochemical model},
  author={Chu, Zhengyu and Feng, Xuning and Lu, Languang and Li, Jianqiu and Han, Xuebing and Ouyang, Minggao},
  journal={Applied Energy},
  year={2017},
  publisher={Elsevier}
}
@article{liu2017extended,
  title={An extended differential flatness approach for the health-conscious nonlinear model predictive control of lithium-ion batteries},
  author={Liu, Ji and Li, Guang and Fathy, Hosam K},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={5},
  pages={1882--1889},
  year={2017},
  publisher={IEEE}
}
@article{fang2017health,
  title={Health-aware and user-involved battery charging management for electric vehicles: Linear quadratic strategies},
  author={Fang, Huazhen and Wang, Yebin and Chen, Jian},
  journal={IEEE Transactions on Control Systems Technology},
  volume={25},
  number={3},
  pages={911--923},
  year={2017},
  publisher={IEEE}
}
@article{methekar2010optimum,
  title={Optimum charging profile for lithium-ion batteries to maximize energy storage and utilization},
  author={Methekar, Ravi and Ramadesigan, Venkatasailanathan and Braatz, Richard D and Subramanian, Venkat R},
  journal={ECS Transactions},
  volume={25},
  number={35},
  pages={139--146},
  year={2010},
  publisher={The Electrochemical Society}
}
@inproceedings{torchio2015real,
  title={Real-time model predictive control for the optimal charging of a lithium-ion battery},
  author={Torchio, Marcello and Wolff, Nicolas A and Raimondo, Davide M and Magni, Lalo and Krewer, Ulrike and Gopaluni, R Bushan and Paulson, Joel A and Braatz, Richard D},
  booktitle={American Control Conference (ACC), 2015},
  pages={4536--4541},
  year={2015},
  organization={IEEE}
}
@inproceedings{klein2011optimal,
  title={Optimal charging strategies in lithium-ion battery},
  author={Klein, Reinhardt and Chaturvedi, Nalin A and Christensen, Jake and Ahmed, Jasim and Findeisen, Rolf and Kojic, Aleksandar},
  booktitle={American Control Conference (ACC), 2011},
  pages={382--387},
  year={2011},
  organization={IEEE}
}
@article{hu2013charging,
  title={Charging time and loss optimization for LiNMC and LiFePO 4 batteries based on equivalent circuit models},
  author={Hu, Xiaosong and Li, Shengbo and Peng, Huei and Sun, Fengchun},
  journal={Journal of Power Sources},
  volume={239},
  pages={449--457},
  year={2013},
  publisher={Elsevier}
}
@article{perez2017optimal,
  title={Optimal Charging of Li-Ion Batteries via a Single Particle Model with Electrolyte and Thermal Dynamics},
  author={Perez, HE and Dey, S and Hu, X and Moura, SJ},
  journal={Journal of The Electrochemical Society},
  volume={164},
  number={7},
  pages={A1679--A1687},
  year={2017},
  publisher={The Electrochemical Society}
}
@article{zou2017electrothermal,
  title={Electrothermal dynamics-conscious lithium-ion battery cell-level charging management via state-monitored predictive control},
  author={Zou, Changfu and Hu, Xiaosong and Wei, Zhongbao and Tang, Xiaolin},
  journal={Energy},
  volume={141},
  pages={250--259},
  year={2017},
  publisher={Elsevier}
}
@article{perez2017optimal2,
  title={Optimal Charging of Li-Ion Batteries with Coupled Electro-Thermal-Aging Dynamics},
  author={Perez, Hector and Hu, Xiaosong and Dey, Satadru and Moura, Scott},
  journal={IEEE Transactions on Vehicular Technology},
  year={2017},
  publisher={IEEE}
}
@article{zou2016modelling,
  title={Modelling, State Estimation \& Optimal Charging Control for A Lithium-Ion Battery},
  author={Zou, Changfu},
  year={2016}
}
@article{bernardi1985general,
  title={A general energy balance for battery systems},
  author={Bernardi, D and Pawlikowski, E and Newman, John},
  journal={Journal of the electrochemical society},
  volume={132},
  number={1},
  pages={5--12},
  year={1985},
  publisher={The Electrochemical Society}
}
@article{doughty2012general,
  title={A general discussion of Li ion battery safety},
  author={Doughty, Daniel H and Roth, E Peter},
  journal={The Electrochemical Society Interface},
  volume={21},
  number={2},
  pages={37--44},
  year={2012},
  publisher={The Electrochemical Society}
}



@ARTICLE{Bandhauer2011,
author = {Bandhauer, Todd M. and Garimella, Srinivas and Fuller, Thomas F.}, 
title = {A Critical Review of Thermal Issues in Lithium-Ion Batteries},
volume = {158}, 
number = {3}, 
pages = {R1-R25}, 
year = {2011}, 
doi = {10.1149/1.3515880}, 
abstract ={Lithium-ion batteries are well-suited for fully electric and hybrid electric vehicles due to their high specific energy and energy density relative to other rechargeable cell chemistries. However, these batteries have not been widely deployed commercially in these vehicles yet due to safety, cost, and poor low temperature performance, which are all challenges related to battery thermal management. In this paper, a critical review of the available literature on the major thermal issues for lithium-ion batteries is presented. Specific attention is paid to the effects of temperature and thermal management on capacity/power fade, thermal runaway, and pack electrical imbalance and to the performance of lithium-ion cells at cold temperatures. Furthermore, insights gained from previous experimental and modeling investigations are elucidated. These include the need for more accurate heat generation measurements, improved modeling of the heat generation rate, and clarity in the relative magnitudes of the various thermal effects observed at high charge and discharge rates seen in electric vehicle applications. From an analysis of the literature, the requirements for lithium-ion thermal management systems for optimal performance in these applications are suggested, and it is clear that no existing thermal management strategy or technology meets all these requirements.}, 
URL = {http://jes.ecsdl.org/content/158/3/R1.abstract}, 
eprint = {http://jes.ecsdl.org/content/158/3/R1.full.pdf+html}, 
journal = {Journal of The Electrochemical Society} 
}

@ARTICLE{Charkhgard2010, 
author={Charkhgard, M. and Farrokhi, M.}, 
journal={Industrial Electronics, IEEE Transactions on}, 
title={State-of-Charge Estimation for Lithium-Ion Batteries Using Neural Networks and EKF}, 
year={2010}, 
volume={57}, 
number={12}, 
pages={4178-4187}, 
keywords={Kalman filters;battery chargers;covariance matrices;neural nets;power engineering computing;secondary cells;battery charging;battery terminal voltage;covariance matrix;extended Kalman filter;lithium-ion batteries;neural networks;state-of-charge estimation;Battery charge measurement;Electrochemical impedance spectroscopy;Impedance measurement;Laboratories;Neural networks;Permission;Pulse power systems;State estimation;Testing;Voltage;Batteries;Kalman filtering;estimation;monitoring;neural networks (NNs)}, 
doi={10.1109/TIE.2010.2043035}, 
ISSN={0278-0046}, 
month={Dec},}

@article{Chen2005,
title = "Thermal analysis of lithium-ion batteries ",
journal = "Journal of Power Sources ",
volume = "140",
number = "1",
pages = "111 - 124",
year = "2005",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2004.05.064",
url = "http://www.sciencedirect.com/science/article/pii/S0378775304008596",
author = "S.C. Chen and C.C. Wan and Y.Y. Wang",
keywords = "Thermal modelling",
keywords = "Thermal analysis",
keywords = "Lithium batteries",
keywords = "Heat dissipation",
keywords = "Thermal management "
}

@article{Debert2013,
title = "An observer looks at the cell temperature in automotive battery packs ",
journal = "Control Engineering Practice ",
volume = "21",
number = "8",
pages = "1035 - 1042",
year = "2013",
note = "",
issn = "0967-0661",
doi = "http://dx.doi.org/10.1016/j.conengprac.2013.03.001",
url = "http://www.sciencedirect.com/science/article/pii/S0967066113000464",
author = "Maxime Debert and Guillaume Colin and Gérard Bloch and Yann Chamaillard",
keywords = "Li-ion battery",
keywords = "Electric Vehicle (EV)",
keywords = "Cell temperature estimation",
keywords = "Internal resistance estimation",
keywords = "Linear Parameter-Varying (LPV) system",
keywords = "Polytopic observer "
}

@ARTICLE{Dey2015a, 
author={Dey, S. and Ayalew, B. and Pisu, P.}, 
journal={Control Systems Technology, IEEE Transactions on}, 
title={Nonlinear Robust Observers for State-of-Charge Estimation of Lithium-Ion Cells Based on a Reduced Electrochemical Model}, 
year={2015}, 
volume={23}, 
number={5}, 
pages={1935-1942}, 
keywords={Lyapunov methods;battery management systems;control system synthesis;linear matrix inequalities;nonlinear control systems;observers;robust control;secondary cells;variable structure systems;Luenberger term design;Lyapunov direct method;SOC information;battery management systems;cell-level state-of-charge information;linear matrix inequality;lithium-ion cells;module-level state-of-charge information;nonlinear robust observers;reduced order electrochemical model;state-of-charge estimation;variable structure term;Electrodes;Integrated circuit modeling;Mathematical model;Observers;System-on-chip;Uncertainty;Electrochemical model;lithium-ion (Li-ion) batteries;nonlinear observer;single-particle model (SPM);state of charge (SOC);state of charge (SOC).}, 
doi={10.1109/TCST.2014.2382635}, 
ISSN={1063-6536}, 
month={Sept},}

@article{Dey2015b,
title = "On-board Thermal Fault Diagnosis of Lithium-ion Batteries For Hybrid Electric Vehicle Application ",
journal = "4th IFAC Workshop on Engine and Powertrain Control, Simulation and Modeling E-COSM 2015",
volume = "48",
number = "15",
pages = "389 - 394",
year = "2015",
note = " ",
issn = "2405-8963",
doi = "http://dx.doi.org/10.1016/j.ifacol.2015.10.056",
url = "http://www.sciencedirect.com/science/article/pii/S2405896315019321",
author = "Satadru Dey and Zoleikha Abdollahi Biron and Sagar Tatipamula and Nabarun Das and Sara Mohon and Beshah Ayalew and Pierluigi Pisu",
keywords = "Lithium-ion Batteries",
keywords = "Fault Diagnosis",
keywords = "Thermal Failure",
keywords = "Observer "
}

@article{Doughty2002,
title = "Lithium battery thermal models ",
journal = "Journal of Power Sources ",
volume = "110",
number = "2",
pages = "357 - 363",
year = "2002",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/S0378-7753(02)00198-2",
url = "http://www.sciencedirect.com/science/article/pii/S0378775302001982",
author = "Daniel H Doughty and Paul C Butler and Rudolph G Jungst and E.Peter Roth",
keywords = "Thermal battery",
keywords = "Lithium-ion cell",
keywords = "Calorimeter",
keywords = "Thermal model",
keywords = "Electrochemical model",
keywords = "Abuse tolerance",
keywords = "Safety "
}

@INPROCEEDINGS{Gould2008, 
author={Gould, C.R. and Bingham, C.M. and Stone, D.A. and Bentley, P.}, 
booktitle={Power Electronics, Electrical Drives, Automation and Motion, 2008. SPEEDAM 2008. International Symposium on}, 
title={Novel battery model of an all-electric personal rapid transit vehicle to determine state-of-health through subspace parameter estimation and a Kalman Estimator}, 
year={2008}, 
pages={1217-1222}, 
keywords={ageing;battery management systems;battery powered vehicles;electrical safety;equivalent circuits;parameter estimation;rapid transit systems;real-time systems;Kalman estimator;Randles model;all-electric personal rapid transit vehicle;battery ageing;equivalent circuit;online monitoring;real-time adaptive battery model;safety-critical system;subspace parameter estimation;Battery powered vehicles;Condition monitoring;Degradation;Equivalent circuits;Fluctuations;Kalman filters;Parameter estimation;State estimation;Temperature;Voltage;Battery management systems;Energy storage;Parameter estimation;System identification}, 
doi={10.1109/SPEEDHAM.2008.4581332}, 
month={June},}

@article{Guo2010,
title = "Three-dimensional thermal finite element modeling of lithium-ion battery in thermal abuse application ",
journal = "Journal of Power Sources ",
volume = "195",
number = "8",
pages = "2393 - 2398",
year = "2010",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2009.10.090",
url = "http://www.sciencedirect.com/science/article/pii/S0378775309019417",
author = "Guifang Guo and Bo Long and Bo Cheng and Shiqiong Zhou and Peng Xu and Binggang Cao",
keywords = "Thermal model",
keywords = "Oven abuse test",
keywords = "Thermal runaway",
keywords = "Lithium-ion battery "
}

@article{Hallaj1999,
title = "Thermal modeling and design considerations of lithium-ion batteries ",
journal = "Journal of Power Sources ",
volume = "83",
number = "1–2",
pages = "1 - 8",
year = "1999",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/S0378-7753(99)00178-0",
url = "http://www.sciencedirect.com/science/article/pii/S0378775399001780",
author = "S. Al Hallaj and H. Maleki and J.S. Hong and J.R. Selman",
keywords = "Thermal modeling",
keywords = "Thermal runaway",
keywords = "Sony cell",
keywords = "Li-ion cells",
keywords = "Scale-up design "
}

@article{Hu2012,
title = "Battery cell state-of-charge estimation using linear parameter varying system techniques ",
journal = "Journal of Power Sources ",
volume = "198",
number = "",
pages = "338 - 350",
year = "2012",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2011.09.058",
url = "http://www.sciencedirect.com/science/article/pii/S0378775311018295",
author = "Y. Hu and S. Yurkovich",
keywords = "Lithium ion batteries",
keywords = "SoC estimation",
keywords = "State estimator",
keywords = "Linear parameter varying systems "
}

@article{Kim2006,
title = "The novel state of charge estimation method for lithium battery using sliding mode observer ",
journal = "Journal of Power Sources ",
volume = "163",
number = "1",
pages = "584 - 590",
year = "2006",
note = "Special issue including selected papers presented at the Second International Conference on Polymer Batteries and Fuel Cells together with regular papers ",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2006.09.006",
url = "http://www.sciencedirect.com/science/article/pii/S0378775306018349",
author = "Il-Song Kim",
keywords = "State of charge estimation",
keywords = "Sliding mode observer",
keywords = "SOC",
keywords = "Lithium battery modeling "
}

@ARTICLE{Kim2014, 
author={Youngki Kim and Mohan, S. and Siegel, J.B. and Stefanopoulou, A.G. and Yi Ding}, 
journal={Control Systems Technology, IEEE Transactions on}, 
title={The Estimation of Temperature Distribution in Cylindrical Battery Cells Under Unknown Cooling Conditions}, 
year={2014}, 
volume={22}, 
number={6}, 
pages={2277-2286}, 
keywords={Kalman filters;battery powered vehicles;cooling;estimation theory;forced convection;hybrid electric vehicles;iron compounds;lithium compounds;nonlinear filters;polynomial approximation;secondary cells;temperature distribution;DKF;LiFePO4;battery core temperature estimation;battery current measurement;cylindrical lithium-iron-phosphate battery cell;dual Kalman filter;extended Kalman filter;forced-air convective cooling;homogeneous volume;hybrid electric vehicle drive cycle;isotropic volume;polynomial approximation;reduced-order thermal model;surface temperature measurement;temperature distribution estimation;unknown cooling condition;voltage measurement;volume averaged lumped-value;Batteries;Battery charge measurement;Kalman filters;Lithium batteries;Parameter estimation;Reduced order systems;State estimation;Temperature distribution;Dual Kalman filter (DKF);lithium ion (Li-ion) batteries;reduced-order model;state and parameter estimation;thermal modeling;thermal modeling.}, 
doi={10.1109/TCST.2014.2309492}, 
ISSN={1063-6536}, 
month={Nov},}


@ARTICLE{Klein2013, 
author={Klein, R. and Chaturvedi, N.A. and Christensen, J. and Ahmed, J. and Findeisen, R. and Kojic, A.}, 
journal={Control Systems Technology, IEEE Transactions on}, 
title={Electrochemical Model Based Observer Design for a Lithium-Ion Battery}, 
year={2013}, 
volume={21}, 
number={2}, 
pages={289-301}, 
keywords={algebra;battery powered vehicles;electric current measurement;observers;partial differential equations;safety;secondary cells;voltage measurement;Li;current measurements;electric-vehicle drive cycles;electrochemical model based observer design;energy storage;internal temperature;lithium-ion battery;mobile electrification;model based controller;optimal operation;output error injection observer;partial differential-algebraic equations;safe operation;safety;state estimation strategy;unmodeled dynamics;voltage measurements;Batteries;Electrodes;Lithium;Mathematical model;Observers;Solids;Battery management systems;PDE observer design;electrochemical model;lithium ion batteries}, 
doi={10.1109/TCST.2011.2178604}, 
ISSN={1063-6536}, 
month={March},}

@ARTICLE{Lin2013, 
author={Xinfan Lin and Perez, H.E. and Siegel, J.B. and Stefanopoulou, A.G. and Yonghua Li and Anderson, R.D. and Yi Ding and Castanier, M.P.}, 
journal={Control Systems Technology, IEEE Transactions on}, 
title={Online Parameterization of Lumped Thermal Dynamics in Cylindrical Lithium Ion Batteries for Core Temperature Estimation and Health Monitoring}, 
year={2013}, 
volume={21}, 
number={5}, 
pages={1745-1755}, 
keywords={condition monitoring;lithium;observers;parameter estimation;secondary cells;temperature measurement;26650 lithium iron phosphate-graphite;Li;adaptive observer;core temperature estimation;cylindrical lithium ion batteries;health monitoring;lumped thermal dynamics;online parameter identification;online parameterization;online parameterization methodology;overheating;surface temperature measurement;temperature-dependent internal resistance;thermal model;thermal monitoring;Adaptation models;Batteries;Battery charge measurement;Coolants;Heating;Resistance;Temperature measurement;Adaptive estimation;core temperature;lithium ion battery;state of health}, 
doi={10.1109/TCST.2012.2217143}, 
ISSN={1063-6536}, 
month={Sept},}

@INPROCEEDINGS{Lombardi2014, 
author={Lombardi, W. and Zarudniev, M. and Lesecq, S. and Bacquet, S.}, 
booktitle={Control Conference (ECC), 2014 European}, 
title={Sensors fault diagnosis for a BMS}, 
year={2014}, 
pages={952-957}, 
keywords={battery management systems;fault diagnosis;sensors;BMS;battery management system;battery pack design;cells;current;sensor faults;sensors fault diagnosis;temperature;voltage;Batteries;Equations;Mathematical model;Temperature measurement;Temperature sensors;Voltage measurement}, 
doi={10.1109/ECC.2014.6862432}, 
month={June},}

@article{Maleki2003,
title = "Thermal analysis and modeling of a notebook computer battery ",
journal = "Journal of Power Sources ",
volume = "115",
number = "1",
pages = "131 - 136",
year = "2003",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/S0378-7753(02)00722-X",
url = "http://www.sciencedirect.com/science/article/pii/S037877530200722X",
author = "Hossein Maleki and Ahmad K Shamsuri",
keywords = "Li-ion cells",
keywords = "Thermal modeling",
keywords = "Computer battery packs "
}

@article{Plett2004,
title = "Extended Kalman filtering for battery management systems of LiPB-based \{HEV\} battery packs: Part 3. State and parameter estimation ",
journal = "Journal of Power Sources ",
volume = "134",
number = "2",
pages = "277 - 292",
year = "2004",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2004.02.033",
url = "http://www.sciencedirect.com/science/article/pii/S0378775304003611",
author = "Gregory L. Plett",
keywords = "Battery management system (BMS)",
keywords = "Hybrid-electric-vehicle (HEV)",
keywords = "Extended Kalman filter (EKF)",
keywords = "State-of-charge (SOC)",
keywords = "State-of-health (SOH)",
keywords = "Lithium-ion polymer battery (LiPB) "
}

@article{Richardson2014,
title = "Battery internal temperature estimation by combined impedance and surface temperature measurement ",
journal = "Journal of Power Sources ",
volume = "265",
number = "",
pages = "254 - 261",
year = "2014",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2014.04.129",
url = "http://www.sciencedirect.com/science/article/pii/S0378775314006302",
author = "Robert R. Richardson and Peter T. Ireland and David A. Howey",
keywords = "Lithium-ion",
keywords = "Electrochemical impedance spectroscopy",
keywords = "Temperature",
keywords = "Thermal runaway",
keywords = "Battery management system "
}

@INPROCEEDINGS{Singh2013, 
author={Singh, A. and Izadian, A. and Anwar, S.}, 
booktitle={Industrial Electronics Society, IECON 2013 - 39th Annual Conference of the IEEE}, 
title={Fault diagnosis of Li-Ion batteries using multiple-model adaptive estimation}, 
year={2013}, 
pages={3524-3529}, 
keywords={Kalman filters;electrochemical impedance spectroscopy;equivalent circuits;fault diagnosis;secondary cells;Kalman filters;battery fault detection unit;battery models;equivalent circuit;fault diagnosis;impedance spectroscopy;model parameter variation;multiple model adaptive estimation;secondary batteries;Adaptation models;Batteries;Circuit faults;Impedance;Integrated circuit modeling;Kalman filters;Mathematical model}, 
doi={10.1109/IECON.2013.6699695}, 
ISSN={1553-572X}, 
month={Nov},}

@ARTICLE{Zhang2002, 
author={Xiaodong Zhang and Polycarpou, M.M. and Parisini, T.}, 
journal={Automatic Control, IEEE Transactions on}, 
title={A robust detection and isolation scheme for abrupt and incipient faults in nonlinear systems}, 
year={2002}, 
volume={47}, 
number={4}, 
pages={576-593}, 
keywords={fault diagnosis;nonlinear control systems;nonlinear dynamical systems;robust control;state estimation;uncertain systems;abrupt faults;adaptive residual threshold;fault isolability conditions;incipient faults;isolation estimators;nonlinear adaptive estimator;nonlinear uncertain dynamic systems;online health monitoring;robust detection and isolation scheme;robust fault diagnosis;simulation examples;Algorithm design and analysis;Equations;Fault detection;Fault diagnosis;Monitoring;Nonlinear systems;Robustness;State estimation;Uncertain systems;Uncertainty}, 
doi={10.1109/9.995036}, 
ISSN={0018-9286}, 
month={Apr},}

@ARTICLE{Dey2015c,
  author  = {S. Dey and B. Ayalew and P. Pisu}, 
  title   = {Nonlinear Adaptive Observer for a Lithium-ion Battery Cell Based on Coupled Electrochemical-Thermal Model},
  journal = {ASME Journal of Dynamic Systems, Measurement, and Control},
  year    = {2015},
volume  = {137},
  number  = {11},
  pages   = {111005},
  }

@ARTICLE{Moura2014,
  title={Adaptive partial differential equation observer for battery state-of-charge/state-of-health estimation via an electrochemical model},
  author={Moura, Scott J and Chaturvedi, Nalin A and Krsti{\'c}, Miroslav},
  journal={ASME Journal of Dynamic Systems, Measurement, and Control},
  volume={136},
  number={1},
  pages={011015},
  year={2014},
  publisher={American Society of Mechanical Engineers}
}
	
	@article{Dey2017acc,
  author  = {S. Dey and H. E. Perez and Scott  Moura}, 
  title   = {Thermal Fault Diagnostics in Lithium-ion Batteries based on a Distributed Parameter Thermal Model},
	note    = {submitted to American Control Conference 2017, available online http://escholarship.org/uc/item/17q3977b},
  }
	
	@INPROCEEDINGS{Dey2015e,
  author       = {S. Dey and B. Ayalew}, 
  title        = {A Diagnostic Scheme for Detection, Isolation and Estimation of Electrochemical Faults in Lithium-Ion Cells},
  booktitle    = {2014 ASME Dynamic Systems and Control Conference (DSCC)},
  year         = 2014,
  editor       = {},
  volume       = 4,
  series       = 5,
  pages        = V001T13A001,
  address      = {},
  month        = {},
  organization = {},
  publisher    = {},
  note         = {}  
}

@inproceedings{Marcicki2010,
  title={Nonlinear fault detection and isolation for a lithium-ion battery management system},
  author={Marcicki, Jim and Onori, Simona and Rizzoni, Giorgio},
  booktitle={ASME 2010 Dynamic Systems and Control Conference},
  pages={607--614},
  year={2010},
  organization={American Society of Mechanical Engineers}
}

@inproceedings{liu2014,
  title={Fault detection and isolation for lithium-ion battery system using structural analysis and sequential residual generation},
  author={Liu, Zhentong and Ahmed, Qadeer and Rizzoni, Giorgio and He, Hongwen},
  booktitle={ASME 2014 Dynamic Systems and Control Conference},
  pages={V002T36A005--V002T36A005},
  year={2014},
  organization={American Society of Mechanical Engineers}
}

@article{Mukhopadhyay2014,
title = "A high-gain adaptive observer for detecting Li-ion battery terminal voltage collapse ",
journal = "Automatica ",
volume = "50",
number = "3",
pages = "896 - 902",
year = "2014",
note = "",
issn = "0005-1098",
doi = "http://dx.doi.org/10.1016/j.automatica.2013.12.011",
url = "http://www.sciencedirect.com/science/article/pii/S0005109813005700",
author = "Shayok Mukhopadhyay and Fumin Zhang",
keywords = "Adaptive systems",
keywords = "Adaptive filters",
keywords = "Detection algorithms",
keywords = "High-gain",
keywords = "Trend "
}


@article{lopez2015experimental,
  title={Experimental Analysis of Thermal Runaway and Propagation in Lithium-Ion Battery Modules},
  author={Lopez, Carlos F and Jeevarajan, Judith A and Mukherjee, Partha P},
  journal={Journal of The Electrochemical Society},
  volume={162},
  number={9},
  pages={A1905--A1915},
  year={2015},
  publisher={The Electrochemical Society}
}
@book{lewis2007optimal,
  title={Optimal and robust estimation: with an introduction to stochastic control theory},
  author={Lewis, Frank L and Xie, Lihua and Popa, Dan},
  volume={29},
  year={2007},
  publisher={CRC press}
}
@book{utkin2009sliding,
  title={Sliding mode control in electro-mechanical systems},
  author={Utkin, Vadim and Guldner, J{\"u}rgen and Shi, Jingxin},
  volume={34},
  year={2009},
  publisher={CRC press}
}
@book{isidori,
  title={Nonlinear Control Systems II},
  author={Isidori, Alberto },
  year={1999},
  publisher={Springer}
}

@article{Lin20141,
title = "A lumped-parameter electro-thermal model for cylindrical batteries ",
journal = "Journal of Power Sources ",
volume = "257",
number = "",
pages = "1 - 11",
year = "2014",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2014.01.097",
url = "http://www.sciencedirect.com/science/article/pii/S0378775314001244",
author = "Xinfan Lin and Hector E. Perez and Shankar Mohan and Jason B. Siegel and Anna G. Stefanopoulou and Yi Ding and Matthew P. Castanier",
keywords = "Lithium ion batteries",
keywords = "Electro-thermal model",
keywords = "Parameterization",
keywords = "Core temperature",
keywords = "State of charge "
}

@book{krstic2008boundary,
  title={Boundary control of PDEs: A course on backstepping designs},
  author={Krstic, Miroslav and Smyshlyaev, Andrey},
  volume={16},
  year={2008},
  publisher={Siam}
}

@book{cengel2011,
  title={Heat and Mass Transfer: Fundamentals and Applications, 5e},
  author={Yunus A. Cengel and Afshin J. Ghajar},
  volume={},
  year={2011},
  publisher={McGraw-Hill}
}

@article{Dey201637,
title = "Model-based real-time thermal fault diagnosis of Lithium-ion batteries ",
journal = "Control Engineering Practice ",
volume = "56",
number = "",
pages = "37 - 48",
year = "2016",
note = "",
issn = "0967-0661",
doi = "http://dx.doi.org/10.1016/j.conengprac.2016.08.002",
url = "http://www.sciencedirect.com/science/article/pii/S0967066116301654",
author = "Satadru Dey and Zoleikha Abdollahi Biron and Sagar Tatipamula and Nabarun Das and Sara Mohon and Beshah Ayalew and Pierluigi Pisu",
keywords = "Lithium-ion batteries",
keywords = "Fault diagnosis",
keywords = "Thermal faults",
keywords = "Observer",
keywords = "Adaptive threshold "
}

@article{Fang20141090,
title = "Study of internal short in a Li-ion cell-II. Numerical investigation using a 3D electrochemical-thermal model ",
journal = "Journal of Power Sources ",
volume = "248",
number = "",
pages = "1090 - 1098",
year = "2014",
note = "",
issn = "0378-7753",
doi = "http://dx.doi.org/10.1016/j.jpowsour.2013.10.004",
url = "http://www.sciencedirect.com/science/article/pii/S0378775313016546",
author = "Weifeng Fang and Premanand Ramadass and Zhengming (John) Zhang",
keywords = "Li-ion cell",
keywords = "Internal short circuit",
keywords = "3D",
keywords = "Electrochemical-thermal",
keywords = "Model "
}


@ARTICLE{Motapon2016, 
author={S. N. Motapon and A. Lupien-Bedard and L. A. Dessaint and H. Fortin-Blanchette and K. Al-Haddad}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={A Generic Electro-Thermal Li-Ion Battery Model for Rapid Evaluation of Cell Temperature Temporal Evolution}, 
year={2016}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Batteries;Data models;Discharges (electric);Integrated circuit modeling;Mathematical model;Thermal resistance;CC-CV charging;Li-ion batteries;electrical simulation;electro-thermal modelling;generic battery model;least-square algorithm}, 
doi={10.1109/TIE.2016.2618363}, 
ISSN={0278-0046}, 
month={},}

@ARTICLE{Zhang2016tie, 
author={C. Zhang and K. Li and J. Deng and S. Song}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={Improved Real-time State-of-Charge Estimation of LiFePO4 Battery Based on a Novel Thermoelectric Model}, 
year={2016}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Batteries;Estimation;Heating;Integrated circuit modeling;State of charge;Temperature;Temperature measurement;Internal temperature estimation;SOC estimation;joint extended Kalman Filter;thermoelectric model}, 
doi={10.1109/TIE.2016.2610398}, 
ISSN={0278-0046}, 
month={},}

@ARTICLE{Mejdoubi2016, 
author={A. El Mejdoubi and A. Oukaour and H. Chaoui and H. Gualous and J. Sabor and Y. Slamani}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={State-of-Charge and State-of-Health Lithium-Ion Batteries Diagnosis According to Surface Temperature Variation}, 
year={2016}, 
volume={63}, 
number={4}, 
pages={2391-2402}, 
keywords={Kalman filters;Lyapunov methods;nonlinear filters;secondary cells;EKF;Lyapunov direct method;SOC;SOH;STV;extended Kalman filter;lithium-ion batteries;state-of-charge;state-of-health estimation technique;surface temperature variation;Aging;Batteries;Discharges (electric);Estimation;Kalman filters;Resistance;Temperature measurement;Adaptive observer;Extended Kalman Filter;Lithium-ion batteries;Lyapunov stability;Parameters estimation;State-of-Charge;State-of-Health;extended Kalman filter (EKF);lithium-ion batteries;parameters estimation;state-of-charge (SOC);state-of-health (SOH)}, 
doi={10.1109/TIE.2015.2509916}, 
ISSN={0278-0046}, 
month={April},}

@ARTICLE{Sidhu2015tie, 
author={A. Sidhu and A. Izadian and S. Anwar}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={Adaptive Nonlinear Model-Based Fault Diagnosis of Li-Ion Batteries}, 
year={2015}, 
volume={62}, 
number={2}, 
pages={1002-1011}, 
keywords={equivalent circuits;fault diagnosis;iron compounds;lithium compounds;nonlinear filters;phosphorus compounds;secondary cells;Li-ion batteries;LiFePO4;equivalent circuit methodology;extended Kalman filters;fault diagnosis technique;impedance spectroscopy;multiple-model adaptive estimation technique;nonlinear battery signature-fault models;parameter variation;residual signals;terminal voltage;Adaptation models;Batteries;Circuit faults;Equivalent circuits;Fault diagnosis;Impedance;Integrated circuit modeling;Extended Kalman filter (EKF);Li-ion battery;fault diagnosis;multiple-model adaptive fault diagnosis}, 
doi={10.1109/TIE.2014.2336599}, 
ISSN={0278-0046}, 
month={Feb},}

@ARTICLE{Rahimi2014tie, 
author={H. Rahimi-Eichi and F. Baronti and M. Y. Chow}, 
journal={IEEE Transactions on Industrial Electronics}, 
title={Online Adaptive Parameter Identification and State-of-Charge Coestimation for Lithium-Polymer Battery Cells}, 
year={2014}, 
volume={61}, 
number={4}, 
pages={2053-2061}, 
keywords={RC circuits;battery charge measurement;estimation theory;least squares approximations;parameter estimation;piecewise linear techniques;secondary cells;RC equivalent circuit;RC parameters;SOC coestimation method;battery dynamics;charging-discharging rates;estimation algorithm;lithium-polymer batteries;moving window least squares parameter-identification technique;nonupdating parameters;open-circuit voltage;piecewise linear approximation with;plug-in hybrid electric vehicles;real-time estimation;resistance-capacitance equivalent circuit;smart grid applications;state of charge;Battery modeling;observer;open-circuit voltage;parameter identification;piecewise linearization;state-of-charge (SOC) estimation}, 
doi={10.1109/TIE.2013.2263774}, 
ISSN={0278-0046}, 
month={April},}


@ARTICLE{Dey2016tcst, 
author={S. Dey and S. Mohon and P. Pisu and B. Ayalew}, 
journal={IEEE Transactions on Control Systems Technology}, 
title={Sensor Fault Detection, Isolation, and Estimation in Lithium-Ion Batteries}, 
year={2016}, 
volume={24}, 
number={6}, 
pages={2141-2149}, 
keywords={Batteries;Battery management systems;Fault detection;Lithium batteries;Observers;Temperature sensors;Fault detection and isolation;Li-ion batteries;fault estimation;sensor fault;sliding mode observers}, 
doi={10.1109/TCST.2016.2538200}, 
ISSN={1063-6536}, 
month={Nov},}

@article{forgez2010thermal,
  title={Thermal modeling of a cylindrical LiFePO 4/graphite lithium-ion battery},
  author={Forgez, Christophe and Do, Dinh Vinh and Friedrich, Guy and Morcrette, Mathieu and Delacourt, Charles},
  journal={Journal of Power Sources},
  volume={195},
  number={9},
  pages={2961--2968},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{biron2015observer,
  title={Observer-Based Diagnostic Scheme for Lithium-Ion Batteries},
  author={Biron, Zoleikha Abdollahi and Pisu, Pierluigi and Ayalew, Beshah},
  booktitle={ASME 2015 Dynamic Systems and Control Conference},
  pages={V002T19A003--V002T19A003},
  year={2015},
  organization={American Society of Mechanical Engineers}
}


@article{santhanagopalan2009analysis,
  title={Analysis of internal short-circuit in a lithium ion cell},
  author={Santhanagopalan, Shriram and Ramadass, Premanand and Zhang, John Zhengming},
  journal={Journal of Power Sources},
  volume={194},
  number={1},
  pages={550--557},
  year={2009},
  publisher={Elsevier}
}

@article{nguyen2019optimal,
  title={Optimal operation of transmission power networks by using improved stochastic fractal search algorithm},
  author={Nguyen, Thang Trung and Nguyen, Thuan Thanh and Duong, Minh Quan and Doan, Anh Tuan},
  journal={Neural Computing and Applications},
  pages={1--36},
  year={2019},
  publisher={Springer}
}

@article{duong2020optimal,
  title={Optimal Reactive Power Flow for Large-Scale Power Systems Using an Effective Metaheuristic Algorithm},
  author={Duong, Thanh Long and Duong, Minh Quan and Phan, Van-Duc and Nguyen, Thang Trung},
  journal={Journal of Electrical and Computer Engineering},
  volume={2020},
  year={2020},
  publisher={Hindawi}
}

@inbook{inbook1,
	author		= {F. N. Author},
	title			= {Title of the book},
	chapter		= 8,
	pages        = {201-213},
	publisher    = {The name of the publisher},
	year         = 1993,
	volume       = 4,
	series       = {series 1},
	address      = {The address of the publisher},
	edition      = 3,
	month        = {April},
	note         = {An optional note}
}

@book{book1,
	author    = {Full Name Author},
	title     = {Title of the book},
	year      = {1993},
	volume    = 4,
	series    = 10,
	address   = {Country},
	publisher = {The name of the publisher},
	edition   = 3,
	month     = {April},
	note      = {An optional note}
}

@book{onlinebook1,
	title={The title of the online book},
	author={Full Name Author},
	publisher={P. Name},
	isbn={2000000000000},
	lccn={200000000},
	series={Example series},
	url={http://books.google.es},
	month     = {April},	
	year={2003},
}

@article{article1,
	author={Full Name Author1 and F. N. Author2 and Full Name Author3},
	journal={Other Journal},
	title={The title of the article},
	year={1990},
	month= {March},
	volume={IA-21},
	number={4},
	pages={814-821},
	keywords={},
	doi={XX/XXXX/ZZZ.XXXX.XXXXXXX},
	}
	
@ARTICLE{article2,
	author={Full Name Author1},
	journal={Journal title},
	title={The title of the article},
	year={2009},
	volume={56},
	number={2},
	pages={581-588},
	keywords={},
	month={Feb},
	doi={XX/XXXX/ZZZ.XXXX.XXXXXXX},}
	
@INPROCEEDINGS{inproceedings1,
	author={Full Name Author1 and Full Name Author2},
	booktitle={Title of the Proceeding},
	title={The title of the conference},
	year={2003},
	month = {April},
	volume={3},
	pages={1-6},
	keywords={},
	doi={XX/XXXX/ZZZ.XXXX.XXXXXXX},}

@article{patent1,
	author={Full Name Author1 and Full Name Author2 and Full Name Author3},
	title="The title of the patent",
	journal={Jounal Name},
	year={1990},
	month= {Oct},
	number={146643245}
}


%-------------------------------------------------------------------------------------
%----------------------------------------Types----------------------------------------
%-------------------------------------------------------------------------------------
% article
                %An article from a journal or magazine.
% book
                %A book with an explicit publisher.
% booklet
                %A work that is printed and bound, but without a named publisher or sponsoring institution.
% ceedings
                %An article in a conference proceedings.
% proceedings
                %The proceedings of a conference.
% conference
                %The same as inproceedings.
% inbook
                %A part of a book, which may be a chapter (or section or whatever) and/or a range of pages.
% incollection
                %A part of a book having its own title.
% manual
                %Technical documentation.
% mastersthesis
                %A Master's thesis.
% misc
                %Use this type when nothing else fits.
% phdthesis
                %A PhD thesis.
% techreport
                %A report published by a school or other institution, usually numbered within a series.
% unpublished
                %A document having an author and title, but not formally published.
% collection
                %A collection of works. The same as proceedings
% patent
                %A patent.

%-------------------------------------------------------------------------------------
%----------------------------------------Fields---------------------------------------
%-------------------------------------------------------------------------------------
%address
                %Usually the address of the publisher or other type of institution.
%annote
                %An annotation. It is not used by the standard bibliography styles, but may be used by others that produce an annotated bibliography.
%author
                %The name(s) of the author(s), in the format described in the LaTeX book.
%booktitle
                %Title of a book, part of which is being cited. See the LaTeX book for how to type titles. For book entries, use the title field instead.
%chapter
                %A chapter (or section or whatever) number.
%crossref
                %The database key of the entry being cross referenced. Any fields that are missing from the current record are inherited from the field being cross referenced.
%edition
                %The edition of a book---for example, ``Second''. This should be an ordinal, and should have the first letter capitalized, as shown here; the standard styles convert to lower case when necessary.
%editor
                %Name(s) of editor(s), typed as indicated in the LaTeX book. If there is also an author field, then the editor field gives the editor of the book or collection in which the reference appears.
%howpublished
                %How something strange has been published. The first word should be capitalized.
%institution
                %The sponsoring institution of a technical report.
%journal
                %A journal name. Abbreviations are provided for many journals.
%key
                %Used for alphabetizing, cross referencing, and creating a label when the ``author'' information is missing. This field should not be confused with the key that appears in the cite command and at the beginning of the database entry.
%month
                %The month in which the work was published or, for an unpublished work, in which it was written. You should use the standard three-letter abbreviation, as described in Appendix B.1.3 of the LaTeX book.
%note
                %Any additional information that can help the reader. The first word should be capitalized.
%number
                %The number of a journal, magazine, technical report, or of a work in a series. An issue of a journal or magazine is usually identified by its volume and number; the organization that issues a technical report usually gives it a number; and sometimes books are given numbers in a named series.
%organization
                %The organization that sponsors a conference or that publishes a manual.
%pages
                %One or more page numbers or range of numbers, such as 42--111 or 7,41,73--97 or 43+(the `+' in this last example indicates pages following that don't form a simple range). To make it easier to maintain Scribe-compatible databases, the standard styles convert a single dash (as in 7-33) to the double dash used in TeX to denote number ranges (as in 7--33).
%publisher
                %The publisher's name.
%school
                %The name of the school where a thesis was written.
%series
                %The name of a series or set of books. When citing an entire book, the the title field gives its title and an optional series field gives the name of a series or multi-volume set in which the book is published.
%title
                %The work's title, typed as explained in the LaTeX book.
%type
                %The type of a technical report---for example, ``Research Note''.
%volume
                %The volume of a journal or multi-volume book.
%year
                %The year of publication or, for an unpublished work, the year it was written. Generally it should consist of four numerals, such as 1984, although the standard styles can handle any year whose last four nonpunctuation characters are numerals, such as `\hbox{(about 1984)}'.
%affiliation
                %The authors affiliation.
%abstract
                %An abstract of the work.
%contents
                %A Table of Contents
%copyright
                %Copyright information.
%ISBN
                %The International Standard Book Number.
%ISSN
                %The International Standard Serial Number. Used to identify a journal.
%keywords
                %Key words used for searching or possibly for annotation.
%language
                %The language the document is in.
%location
                %A location associated with the entry, such as the city in which a conference took place.
%LCCN
                %The Library of Congress Call Number. I've also seen this as lib-congress.
%mrnumber
                %The Mathematical Reviews number.
%price
                %The price of the document.
%size
                %The physical dimensions of a work.
%URL
                %The WWW Universal Resource Locator that points to the item being referenced. This often is used for technical reports to point to the ftp site where the postscript source of the report is located.
@book{3569,
  title = {Gaussian Processes for Machine Learning},
  author = {Rasmussen, CE. and Williams, CKI.},
  pages = {248},
  series = {Adaptive Computation and Machine Learning},
  publisher = {MIT Press},
  organization = {Max-Planck-Gesellschaft},
  school = {Biologische Kybernetik},
  address = {Cambridge, MA, USA},
  month = jan,
  year = {2006},
  month_numeric = {1}
}
@article{yang2018look,
  title={A look into the voltage plateau signal for detection and quantification of lithium plating in lithium-ion cells},
  author={Yang, Xiao-Guang and Ge, Shanhai and Liu, Teng and Leng, Yongjun and Wang, Chao-Yang},
  journal={Journal of Power Sources},
  volume={395},
  pages={251--261},
  year={2018},
  publisher={Elsevier}
}
